Strategyproof Learning: Building Trustworthy User-Generated Datasets

We prove in this paper that, perhaps surprisingly, incentivizing data misreporting is not a fatality. By leveraging a careful design of the loss function, we propose Licchavi, a global and personalized learning framework with provable strategyproofness guarantees. Essentially, we prove that no user can gain much by replying to Licchavi's queries with answers that deviate from their true preferences. Interestingly, Licchavi also promotes the desirable "one person, one unit-force vote" fairness principle. Furthermore, our empirical evaluation of its performance showcases Licchavi's real-world applicability. We believe that our results are critical for the safety of any learning scheme that leverages user-generated data.

==> general_model.tex <==

In the appendix, to study both \vanilla{} and \system{} at once, we consider a generalized global loss, given by
\begin{equation}
    \globalloss{} (\common, \paramfamily{}, \datafamily{}) 
    = \sum_{\node \in [\NODE]} \left( 
        \reglocalweight{} \norm{\paramsub{\node}}{2}^2 
        + \sum_{\varx \in \data{\node}} \lossperinput(\paramsub{\node})
    \right)
    + \sum_{\node \in [\NODE]} \regularization_{\data{\node}} ( \common - \paramsub{\node}),
\end{equation}
where each function $\regularization_{\data{\node}}$ is a regularization function that may depend on the dataset $\data{\node}$.
Typically, in the case of \system{}, the regularization function depends on $\card{\data{\node}}$.

\begin{assumption}
    For any dataset $\data{}$, the function $\regularization_{\data{}}$ is strictly convex, differentiable, $K_{\data{\node}}$-smooth and has its minimum in $0$.
\end{assumption}
